Avant-Satie! Using ERIK to encode task-relevant expressivity into the animation of autonomous social robots

ERIK is an expressive inverse kinematics technique that has been previously presented and evaluated both algorithmically and in a limited user-interaction scenario. It allows autonomous social robots to convey posture-based expressive information while gaze-tracking users. We have developed a new scenario aimed at further validating some of the unsupported claims from the previous scenario. Our experiment features a fully autonomous Adelino robot, and concludes that ERIK can be used to direct a user's choice of actions during execution of a given task, fully through its non-verbal expressive queues.

==> _preamble.tex <==
\usepackage{amsmath}  % AMS mathematical facilities for LaTeX.
\usepackage{amsthm}   % Typesetting theorems (AMS style).
\usepackage{amsfonts} % 
\usepackage{amssymb}
\usepackage{mathtools}

\usepackage{graphicx}
%\usepackage[pdftex]{hyperref}
\usepackage{multirow}
\usepackage{booktabs}
%\usepackage{subfigure}
\usepackage{subcaption}

\usepackage{etoolbox}
\usepackage{ctable}
\usepackage{enumerate}
\usepackage{multicol}

\usepackage{gensymb}
\usepackage{csquotes}
\usepackage{enumitem}
%\usepackage[table]{xcolor}
\usepackage[acronym]{glossaries}
%\usepackage{hyphenat}

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

%\newtoggle{CAMERA}
%\toggletrue{CAMERA}

%\newcommand{\erik}{\iftoggle{CAMERA}{ERIK}{AnonIK}}

\pagenumbering{arabic}
\pagestyle{plain}
\settopmatter{printfolios=true}

%\exhyphenpenalty=10000


\newacronym{hri}{HRI}{Human-Robot Interaction}
\newacronym{cgi}{CGI}{Computer-Graphics}
\newacronym{ai}{AI}{artificial intelligence}
\newacronym{ik}{IK}{inverse kinematics}
\newacronym[longplural={Degrees of Freedom}]{dof}{DoF}{Degree of Freedom}

\hyphenation{ERIK FABRIK Adelino AvantSatie Jacobian C-ERIK C-EBPS C-Control C-Enhanced Networked}

==> tables/tab_avantsatie_objective_comparison.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Tue Sep 24 19:13:30 2019
\begin{table}[ht]
\centering
\setlength\tabcolsep{5pt}
\begin{tabular}{R{1.8cm}llll}
  \hline
 & ERIK-Control & EBPS-Control & Enhanced-Control & ERIK-EBPS \\ 
  \hline
WrongTotal & \cellcolor[rgb]{0.50,1.00,0.58} ($U{=}90.0, \rho{=}0.008*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U{=}93.5, \rho{=}0.011*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U{=}183.5, \rho{=}0.003*$) & ($U{=}170.5, \rho{=}0.770$) \\ 
WrongCold & ($U{=}128.5, \rho{=}0.129$) & ($U{=}118.0, \rho{=}0.068$) & ($U{=}246.5, \rho{=}0.053$) & ($U{=}176.5, \rho{=}0.907$) \\ 
WrongHot & \cellcolor[rgb]{0.50,1.00,0.58} ($U{=}84.5, \rho{=}0.005*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U{=}94.0, \rho{=}0.012*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U{=}178.5, \rho{=}0.002*$) & ($U{=}173.5, \rho{=}0.840$) \\ 
Time & ($t{=}1.676, \rho{=}0.105$) & \cellcolor[rgb]{0.50,1.00,0.58} ($t{=}2.406, \rho{=}0.022*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U{=}242.0, \rho{=}0.044*$) & ($t{=}0.257, \rho{=}0.798$) \\ 
\end{tabular}
\caption{Results of the comparison of means tests on each of the objective measures. Green with an asterisk* marks comparisons which are significantly different.} 
\label{tab:avantsatie_objective_comparison}
\end{table}


%Time
%	1/2 ($t=1.676, $\rho$=0.105$)
%	3/2 \cellcolor[rgb]{0.50,1.00,0.58} ($t=2.406, $\rho$=0.022*$)
%	4/2 \cellcolor[rgb]{0.50,1.00,0.58} ($U=242.0, $\rho$=0.044*$)
%	1/3 ($t$=0.257, $\rho$=0.798$)

%1		($M=661.0, SD=205.3)
%2		($M=572.2, SD=105.9)
%3		($M=676.2, SD=155.9)
%1+3	($M=668.6, SD=180.0)
%WrongTotal
%	1/2 \cellcolor[rgb]{0.50,1.00,0.58} ($U$=90.0, $\rho$=0.008*$)
%	3/2 \cellcolor[rgb]{0.50,1.00,0.58} ($U$=93.5, $\rho$=0.011*$)
%	4/2 \cellcolor[rgb]{0.50,1.00,0.58} ($U=183.5, \rho=0.003*$)
%	1/3 ($U=170.5, \rho=0.770$)

%1		($M=256.3, SD=132.8)
%2		($M=337.5, SD=109.2)
%3		($M=248.3, SD=92.7)
%1+3	($M=252.3, SD=113.1)
%WrongHot
%	1/2 \cellcolor[rgb]{0.50,1.00,0.58} ($U=84.5, \rho=0.005*$)
%	3/2 \cellcolor[rgb]{0.50,1.00,0.58} ($U=94.0, \rho=0.012*$)
%	4/2 \cellcolor[rgb]{0.50,1.00,0.58} ($U=178.5, \rho=0.002*$)
%	1/3 ($U=173.5, \rho=0.840$)

%1 		($M=117.2, SD=49.9)
%2		($M=161.9, SD=65.4)
%3		($M=122.8, SD=61.0)
%1+3	($M=120.0, SD=55.0)
%WrongCold
%	1/2 ($U=128.5, \rho=0.129$)
%	3/2 ($U=118.0, \rho=0.068$)
%	4/2 ($U=246.5, \rho=0.053$)
%	1/3 ($U=176.5, \rho=0.907$)
%T	($M=141.0, SD=86.1)

==> tables/tab_reliability_analysis.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu Sep 26 11:57:45 2019
\begin{sidewaystable}[ht]
\centering
\begin{tabular}{llllllllllllllllllll}
 Group & ri & rm & cp & pmu & pa & tp & tu & rc & rd & rw & AIL & NM & PA & RC & RD & RIM & RoSAS & RPU & RW \\ 
  \hline
$\alpha_{ALL}$ & \cellcolor[rgb]{0.50,1.00,0.58}0.924 & \cellcolor[rgb]{1.00,0.88,0.30}0.698* & \cellcolor[rgb]{0.50,1.00,0.58}0.745 & \cellcolor[rgb]{0.50,1.00,0.58}0.872 & \cellcolor[rgb]{0.50,1.00,0.58}0.732 & \cellcolor[rgb]{0.50,1.00,0.58}0.749 & \cellcolor[rgb]{1.00,0.88,0.30}0.694* & \cellcolor[rgb]{0.50,1.00,0.58}0.900 & \cellcolor[rgb]{1.00,0.88,0.30}0.648* & \cellcolor[rgb]{0.50,1.00,0.58}0.727 & \cellcolor[rgb]{0.50,1.00,0.58}0.708 & \cellcolor[rgb]{0.50,1.00,0.58}0.870 & \cellcolor[rgb]{0.50,1.00,0.58}0.732 & \cellcolor[rgb]{0.50,1.00,0.58}0.900 & \cellcolor[rgb]{1.00,0.88,0.30}0.648* & \cellcolor[rgb]{0.50,1.00,0.58}0.899 & \cellcolor[rgb]{0.50,1.00,0.58}0.863 & \cellcolor[rgb]{0.50,1.00,0.58}0.731 & \cellcolor[rgb]{0.50,1.00,0.58}0.727 \\ 
  $\omega_{ALL}$ & \cellcolor[rgb]{0.50,1.00,0.58}0.959 & \cellcolor[rgb]{0.50,1.00,0.58}0.759 & \cellcolor[rgb]{0.50,1.00,0.58}0.911 & \cellcolor[rgb]{0.50,1.00,0.58}0.930 & \cellcolor[rgb]{0.50,1.00,0.58}0.785 & \cellcolor[rgb]{0.50,1.00,0.58}0.798 & \cellcolor[rgb]{0.50,1.00,0.58}0.761 & \cellcolor[rgb]{0.50,1.00,0.58}0.938 & \cellcolor[rgb]{0.50,1.00,0.58}0.826 & \cellcolor[rgb]{0.50,1.00,0.58}0.845 & \cellcolor[rgb]{0.50,1.00,0.58}0.721 & \cellcolor[rgb]{0.50,1.00,0.58}0.924 & \cellcolor[rgb]{0.50,1.00,0.58}0.785 & \cellcolor[rgb]{0.50,1.00,0.58}0.938 & \cellcolor[rgb]{0.50,1.00,0.58}0.826 & \cellcolor[rgb]{0.50,1.00,0.58}0.935 & \cellcolor[rgb]{0.50,1.00,0.58}0.908 & \cellcolor[rgb]{0.50,1.00,0.58}0.850 & \cellcolor[rgb]{0.50,1.00,0.58}0.845 \\ 
   \hline
$\alpha_{ERIK}$ & \cellcolor[rgb]{0.50,1.00,0.58}0.929 & \cellcolor[rgb]{1.00,0.88,0.30}0.317* & \cellcolor[rgb]{0.50,1.00,0.58}0.728 & \cellcolor[rgb]{0.50,1.00,0.58}0.788 & \cellcolor[rgb]{0.50,1.00,0.58}0.804 & \cellcolor[rgb]{0.50,1.00,0.58}0.807 & \cellcolor[rgb]{0.50,1.00,0.58}0.775 & \cellcolor[rgb]{0.50,1.00,0.58}0.869 & \cellcolor[rgb]{1.00,0.88,0.30}0.568* & \cellcolor[rgb]{0.50,1.00,0.58}0.772 & \cellcolor[rgb]{1.00,0.88,0.30}0.577* & \cellcolor[rgb]{0.50,1.00,0.58}0.847 & \cellcolor[rgb]{0.50,1.00,0.58}0.804 & \cellcolor[rgb]{0.50,1.00,0.58}0.869 & \cellcolor[rgb]{1.00,0.88,0.30}0.568* & \cellcolor[rgb]{0.50,1.00,0.58}0.887 & \cellcolor[rgb]{0.50,1.00,0.58}0.867 & \cellcolor[rgb]{0.50,1.00,0.58}0.755 & \cellcolor[rgb]{1.00,0.88,0.30}0.626* \\ 
  $\omega_{ERIK}$ & \cellcolor[rgb]{0.50,1.00,0.58}0.971 & \cellcolor[rgb]{1.00,0.88,0.30}0.548* & \cellcolor[rgb]{0.50,1.00,0.58}0.939 & \cellcolor[rgb]{0.50,1.00,0.58}0.898 & \cellcolor[rgb]{0.50,1.00,0.58}0.884 & \cellcolor[rgb]{0.50,1.00,0.58}0.879 & \cellcolor[rgb]{0.50,1.00,0.58}0.912 & \cellcolor[rgb]{0.50,1.00,0.58}0.949 & \cellcolor[rgb]{0.50,1.00,0.58}0.840 & \cellcolor[rgb]{0.50,1.00,0.58}0.891 & \cellcolor[rgb]{1.00,0.88,0.30}0.630* & \cellcolor[rgb]{0.50,1.00,0.58}0.930 & \cellcolor[rgb]{0.50,1.00,0.58}0.884 & \cellcolor[rgb]{0.50,1.00,0.58}0.949 & \cellcolor[rgb]{0.50,1.00,0.58}0.840 & \cellcolor[rgb]{0.50,1.00,0.58}0.935 & \cellcolor[rgb]{0.50,1.00,0.58}0.920 & \cellcolor[rgb]{0.50,1.00,0.58}0.902 & - \\ 
   \hline
$\alpha_{EBPS}$ & \cellcolor[rgb]{0.50,1.00,0.58}0.887 & \cellcolor[rgb]{1.00,0.88,0.30}0.570* & \cellcolor[rgb]{0.50,1.00,0.58}0.881 & \cellcolor[rgb]{0.50,1.00,0.58}0.935 & \cellcolor[rgb]{1.00,0.88,0.30}0.569* & \cellcolor[rgb]{0.50,1.00,0.58}0.846 & \cellcolor[rgb]{1.00,0.88,0.30}0.534* & \cellcolor[rgb]{0.50,1.00,0.58}0.860 & \cellcolor[rgb]{1.00,0.88,0.30}0.405* & \cellcolor[rgb]{0.50,1.00,0.58}0.731 & \cellcolor[rgb]{1.00,0.88,0.30}0.577* & \cellcolor[rgb]{0.50,1.00,0.58}0.891 & \cellcolor[rgb]{1.00,0.88,0.30}0.569* & \cellcolor[rgb]{0.50,1.00,0.58}0.860 & \cellcolor[rgb]{1.00,0.88,0.30}0.405* & \cellcolor[rgb]{0.50,1.00,0.58}0.890 & \cellcolor[rgb]{0.50,1.00,0.58}0.804 & \cellcolor[rgb]{0.50,1.00,0.58}0.744 & \cellcolor[rgb]{0.50,1.00,0.58}0.731 \\ 
  $\omega_{EBPS}$ & \cellcolor[rgb]{0.50,1.00,0.58}0.960 & \cellcolor[rgb]{0.50,1.00,0.58}0.716 & \cellcolor[rgb]{0.50,1.00,0.58}0.969 & \cellcolor[rgb]{0.50,1.00,0.58}0.979 & \cellcolor[rgb]{1.00,0.88,0.30}0.656* & \cellcolor[rgb]{0.50,1.00,0.58}0.754 & \cellcolor[rgb]{0.50,1.00,0.58}0.759 & \cellcolor[rgb]{0.50,1.00,0.58}0.957 & \cellcolor[rgb]{1.00,0.88,0.30}0.495* & \cellcolor[rgb]{0.50,1.00,0.58}0.858 & \cellcolor[rgb]{1.00,0.88,0.30}0.602* & \cellcolor[rgb]{0.50,1.00,0.58}0.956 & \cellcolor[rgb]{1.00,0.88,0.30}0.656* & \cellcolor[rgb]{0.50,1.00,0.58}0.957 & \cellcolor[rgb]{1.00,0.88,0.30}0.495* & \cellcolor[rgb]{0.50,1.00,0.58}0.944 & \cellcolor[rgb]{0.50,1.00,0.58}0.896 & \cellcolor[rgb]{0.50,1.00,0.58}0.907 & \cellcolor[rgb]{0.50,1.00,0.58}0.858 \\ 
   \hline
$\alpha_{Control}$ & \cellcolor[rgb]{0.50,1.00,0.58}0.889 & \cellcolor[rgb]{0.50,1.00,0.58}0.752 & \cellcolor[rgb]{1.00,0.88,0.30}0.636* & \cellcolor[rgb]{0.50,1.00,0.58}0.836 & \cellcolor[rgb]{0.50,1.00,0.58}0.773 & \cellcolor[rgb]{1.00,0.88,0.30}0.540* & \cellcolor[rgb]{0.50,1.00,0.58}0.731 & \cellcolor[rgb]{0.50,1.00,0.58}0.922 & \cellcolor[rgb]{0.50,1.00,0.58}0.748 & \cellcolor[rgb]{1.00,0.88,0.30}0.553* & \cellcolor[rgb]{0.50,1.00,0.58}0.770 & \cellcolor[rgb]{0.50,1.00,0.58}0.835 & \cellcolor[rgb]{0.50,1.00,0.58}0.773 & \cellcolor[rgb]{0.50,1.00,0.58}0.922 & \cellcolor[rgb]{0.50,1.00,0.58}0.748 & \cellcolor[rgb]{0.50,1.00,0.58}0.863 & \cellcolor[rgb]{0.50,1.00,0.58}0.871 & \cellcolor[rgb]{0.50,1.00,0.58}0.728 & \cellcolor[rgb]{1.00,0.88,0.30}0.553* \\ 
  $\omega_{Control}$ & \cellcolor[rgb]{0.50,1.00,0.58}0.943 & \cellcolor[rgb]{0.50,1.00,0.58}0.857 & \cellcolor[rgb]{0.50,1.00,0.58}0.828 & \cellcolor[rgb]{0.50,1.00,0.58}0.903 & \cellcolor[rgb]{0.50,1.00,0.58}0.795 & \cellcolor[rgb]{1.00,0.88,0.30}0.667* & \cellcolor[rgb]{0.50,1.00,0.58}0.825 & \cellcolor[rgb]{0.50,1.00,0.58}0.973 & \cellcolor[rgb]{0.50,1.00,0.58}0.939 & \cellcolor[rgb]{0.50,1.00,0.58}0.768 & \cellcolor[rgb]{0.50,1.00,0.58}0.779 & \cellcolor[rgb]{0.50,1.00,0.58}0.914 & \cellcolor[rgb]{0.50,1.00,0.58}0.795 & \cellcolor[rgb]{0.50,1.00,0.58}0.973 & \cellcolor[rgb]{0.50,1.00,0.58}0.939 & \cellcolor[rgb]{0.50,1.00,0.58}0.925 & \cellcolor[rgb]{0.50,1.00,0.58}0.906 & \cellcolor[rgb]{0.50,1.00,0.58}0.853 & \cellcolor[rgb]{0.50,1.00,0.58}0.768 \\ 
   \hline
$\alpha_{Enhanced}$ & \cellcolor[rgb]{0.50,1.00,0.58}0.908 & \cellcolor[rgb]{1.00,0.88,0.30}0.414* & \cellcolor[rgb]{0.50,1.00,0.58}0.791 & \cellcolor[rgb]{0.50,1.00,0.58}0.867 & \cellcolor[rgb]{1.00,0.88,0.30}0.698* & \cellcolor[rgb]{0.50,1.00,0.58}0.828 & \cellcolor[rgb]{1.00,0.88,0.30}0.678* & \cellcolor[rgb]{0.50,1.00,0.58}0.864 & \cellcolor[rgb]{1.00,0.88,0.30}0.441* & \cellcolor[rgb]{0.50,1.00,0.58}0.750 & \cellcolor[rgb]{1.00,0.88,0.30}0.559* & \cellcolor[rgb]{0.50,1.00,0.58}0.866 & \cellcolor[rgb]{1.00,0.88,0.30}0.698* & \cellcolor[rgb]{0.50,1.00,0.58}0.864 & \cellcolor[rgb]{1.00,0.88,0.30}0.441* & \cellcolor[rgb]{0.50,1.00,0.58}0.857 & \cellcolor[rgb]{0.50,1.00,0.58}0.826 & \cellcolor[rgb]{0.50,1.00,0.58}0.728 & \cellcolor[rgb]{0.50,1.00,0.58}0.750 \\ 
  $\omega_{Enhanced}$ & \cellcolor[rgb]{0.50,1.00,0.58}0.961 & \cellcolor[rgb]{1.00,0.88,0.30}0.599* & \cellcolor[rgb]{0.50,1.00,0.58}0.923 & \cellcolor[rgb]{0.50,1.00,0.58}0.935 & \cellcolor[rgb]{0.50,1.00,0.58}0.773 & \cellcolor[rgb]{0.50,1.00,0.58}0.866 & \cellcolor[rgb]{1.00,0.88,0.30}0.172* & \cellcolor[rgb]{0.50,1.00,0.58}0.928 & \cellcolor[rgb]{1.00,0.88,0.30}0.604* & \cellcolor[rgb]{0.50,1.00,0.58}0.873 & \cellcolor[rgb]{1.00,0.88,0.30}0.606* & \cellcolor[rgb]{0.50,1.00,0.58}0.923 & \cellcolor[rgb]{0.50,1.00,0.58}0.773 & \cellcolor[rgb]{0.50,1.00,0.58}0.928 & \cellcolor[rgb]{1.00,0.88,0.30}0.604* & \cellcolor[rgb]{0.50,1.00,0.58}0.911 & \cellcolor[rgb]{0.50,1.00,0.58}0.886 & \cellcolor[rgb]{0.50,1.00,0.58}0.861 & \cellcolor[rgb]{0.50,1.00,0.58}0.873 \\ 
   \hline
\end{tabular}
\caption{Reliability analysis of the various scales and dimensions, using Cronbach's alpha ($\alpha$) and McDonald's omega ($\omega$). Green represents a \textit{reliable} scale, while yellow with an asterisk* represents otherwise.} 
\end{sidewaystable}


==> tables/tab_reliability_analysis_transp_header.tex <==
%  \input{tab_reliability_analysis_transp_header}
Group & \multicolumn{2}{c}{ALL} & \multicolumn{2}{c}{C-ERIK} & \multicolumn{2}{c}{C-EBPS} & \multicolumn{2}{c}{C-Control} & \multicolumn{2}{c}{C-Enhanced} \\ \hline
& $\alpha$ & $\omega$ & $\alpha$ & $\omega$& $\alpha$ & $\omega$& $\alpha$ & $\omega$& $\alpha$ & $\omega$ \\ 

==> tables/tab_reliability_analysis_transposed.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu Sep 26 11:57:45 2019
\begin{table}[ht]
\centering
\begin{tabular}{rll|ll|ll|ll|ll}
  \toprule
  \input{tables/tab_reliability_analysis_transp_header}
 AIL & \cellcolor[rgb]{0.50,1.00,0.58}0.708 & \cellcolor[rgb]{0.50,1.00,0.58}0.721 & \cellcolor[rgb]{1.00,0.88,0.30}0.577* & \cellcolor[rgb]{1.00,0.88,0.30}0.630* & \cellcolor[rgb]{1.00,0.88,0.30}0.577* & \cellcolor[rgb]{1.00,0.88,0.30}0.602* & \cellcolor[rgb]{0.50,1.00,0.58}0.770 & \cellcolor[rgb]{0.50,1.00,0.58}0.779 & \cellcolor[rgb]{1.00,0.88,0.30}0.559* & \cellcolor[rgb]{1.00,0.88,0.30}0.606* \\ 
  RIM & \cellcolor[rgb]{0.50,1.00,0.58}0.899 & \cellcolor[rgb]{0.50,1.00,0.58}0.935 & \cellcolor[rgb]{0.50,1.00,0.58}0.887 & \cellcolor[rgb]{0.50,1.00,0.58}0.935 & \cellcolor[rgb]{0.50,1.00,0.58}0.890 & \cellcolor[rgb]{0.50,1.00,0.58}0.944 & \cellcolor[rgb]{0.50,1.00,0.58}0.863 & \cellcolor[rgb]{0.50,1.00,0.58}0.925 & \cellcolor[rgb]{0.50,1.00,0.58}0.857 & \cellcolor[rgb]{0.50,1.00,0.58}0.911 \\ 
  RPU & \cellcolor[rgb]{0.50,1.00,0.58}0.731 & \cellcolor[rgb]{0.50,1.00,0.58}0.850 & \cellcolor[rgb]{0.50,1.00,0.58}0.755 & \cellcolor[rgb]{0.50,1.00,0.58}0.902 & \cellcolor[rgb]{0.50,1.00,0.58}0.744 & \cellcolor[rgb]{0.50,1.00,0.58}0.907 & \cellcolor[rgb]{0.50,1.00,0.58}0.728 & \cellcolor[rgb]{0.50,1.00,0.58}0.853 & \cellcolor[rgb]{0.50,1.00,0.58}0.728 & \cellcolor[rgb]{0.50,1.00,0.58}0.861 \\ 
  NM & \cellcolor[rgb]{0.50,1.00,0.58}0.870 & \cellcolor[rgb]{0.50,1.00,0.58}0.924 & \cellcolor[rgb]{0.50,1.00,0.58}0.847 & \cellcolor[rgb]{0.50,1.00,0.58}0.930 & \cellcolor[rgb]{0.50,1.00,0.58}0.891 & \cellcolor[rgb]{0.50,1.00,0.58}0.956 & \cellcolor[rgb]{0.50,1.00,0.58}0.835 & \cellcolor[rgb]{0.50,1.00,0.58}0.914 & \cellcolor[rgb]{0.50,1.00,0.58}0.866 & \cellcolor[rgb]{0.50,1.00,0.58}0.923 \\ 
  PA & \cellcolor[rgb]{0.50,1.00,0.58}0.732 & \cellcolor[rgb]{0.50,1.00,0.58}0.785 & \cellcolor[rgb]{0.50,1.00,0.58}0.804 & \cellcolor[rgb]{0.50,1.00,0.58}0.884 & \cellcolor[rgb]{1.00,0.88,0.30}0.569* & \cellcolor[rgb]{1.00,0.88,0.30}0.656* & \cellcolor[rgb]{0.50,1.00,0.58}0.773 & \cellcolor[rgb]{0.50,1.00,0.58}0.795 & \cellcolor[rgb]{1.00,0.88,0.30}0.698* & \cellcolor[rgb]{0.50,1.00,0.58}0.773 \\ 
  RW & \cellcolor[rgb]{0.50,1.00,0.58}0.727 & \cellcolor[rgb]{0.50,1.00,0.58}0.845 & \cellcolor[rgb]{1.00,0.88,0.30}0.626* & - & \cellcolor[rgb]{0.50,1.00,0.58}0.731 & \cellcolor[rgb]{0.50,1.00,0.58}0.858 & \cellcolor[rgb]{1.00,0.88,0.30}0.553* & \cellcolor[rgb]{0.50,1.00,0.58}0.768 & \cellcolor[rgb]{0.50,1.00,0.58}0.750 & \cellcolor[rgb]{0.50,1.00,0.58}0.873 \\ 
  RC & \cellcolor[rgb]{0.50,1.00,0.58}0.900 & \cellcolor[rgb]{0.50,1.00,0.58}0.938 & \cellcolor[rgb]{0.50,1.00,0.58}0.869 & \cellcolor[rgb]{0.50,1.00,0.58}0.949 & \cellcolor[rgb]{0.50,1.00,0.58}0.860 & \cellcolor[rgb]{0.50,1.00,0.58}0.957 & \cellcolor[rgb]{0.50,1.00,0.58}0.922 & \cellcolor[rgb]{0.50,1.00,0.58}0.973 & \cellcolor[rgb]{0.50,1.00,0.58}0.864 & \cellcolor[rgb]{0.50,1.00,0.58}0.928 \\ 
  RD & \cellcolor[rgb]{1.00,0.88,0.30}0.648* & \cellcolor[rgb]{0.50,1.00,0.58}0.826 & \cellcolor[rgb]{1.00,0.88,0.30}0.568* & \cellcolor[rgb]{0.50,1.00,0.58}0.840 & \cellcolor[rgb]{1.00,0.88,0.30}0.405* & \cellcolor[rgb]{1.00,0.88,0.30}0.495* & \cellcolor[rgb]{0.50,1.00,0.58}0.748 & \cellcolor[rgb]{0.50,1.00,0.58}0.939 & \cellcolor[rgb]{1.00,0.88,0.30}0.441* & \cellcolor[rgb]{1.00,0.88,0.30}0.604* \\ 
  ri & \cellcolor[rgb]{0.50,1.00,0.58}0.924 & \cellcolor[rgb]{0.50,1.00,0.58}0.959 & \cellcolor[rgb]{0.50,1.00,0.58}0.929 & \cellcolor[rgb]{0.50,1.00,0.58}0.971 & \cellcolor[rgb]{0.50,1.00,0.58}0.887 & \cellcolor[rgb]{0.50,1.00,0.58}0.960 & \cellcolor[rgb]{0.50,1.00,0.58}0.889 & \cellcolor[rgb]{0.50,1.00,0.58}0.943 & \cellcolor[rgb]{0.50,1.00,0.58}0.908 & \cellcolor[rgb]{0.50,1.00,0.58}0.961 \\ 
  rm & \cellcolor[rgb]{1.00,0.88,0.30}0.698* & \cellcolor[rgb]{0.50,1.00,0.58}0.759 & \cellcolor[rgb]{1.00,0.88,0.30}0.317* & \cellcolor[rgb]{1.00,0.88,0.30}0.548* & \cellcolor[rgb]{1.00,0.88,0.30}0.570* & \cellcolor[rgb]{0.50,1.00,0.58}0.716 & \cellcolor[rgb]{0.50,1.00,0.58}0.752 & \cellcolor[rgb]{0.50,1.00,0.58}0.857 & \cellcolor[rgb]{1.00,0.88,0.30}0.414* & \cellcolor[rgb]{1.00,0.88,0.30}0.599* \\ 
  tp & \cellcolor[rgb]{0.50,1.00,0.58}0.749 & \cellcolor[rgb]{0.50,1.00,0.58}0.798 & \cellcolor[rgb]{0.50,1.00,0.58}0.807 & \cellcolor[rgb]{0.50,1.00,0.58}0.879 & \cellcolor[rgb]{0.50,1.00,0.58}0.846 & \cellcolor[rgb]{0.50,1.00,0.58}0.754 & \cellcolor[rgb]{1.00,0.88,0.30}0.540* & \cellcolor[rgb]{1.00,0.88,0.30}0.667* & \cellcolor[rgb]{0.50,1.00,0.58}0.828 & \cellcolor[rgb]{0.50,1.00,0.58}0.866 \\ 
  tu & \cellcolor[rgb]{1.00,0.88,0.30}0.694* & \cellcolor[rgb]{0.50,1.00,0.58}0.761 & \cellcolor[rgb]{0.50,1.00,0.58}0.775 & \cellcolor[rgb]{0.50,1.00,0.58}0.912 & \cellcolor[rgb]{1.00,0.88,0.30}0.534* & \cellcolor[rgb]{0.50,1.00,0.58}0.759 & \cellcolor[rgb]{0.50,1.00,0.58}0.731 & \cellcolor[rgb]{0.50,1.00,0.58}0.825 & \cellcolor[rgb]{1.00,0.88,0.30}0.678* & \cellcolor[rgb]{1.00,0.88,0.30}0.172* \\ 
  cp & \cellcolor[rgb]{0.50,1.00,0.58}0.745 & \cellcolor[rgb]{0.50,1.00,0.58}0.911 & \cellcolor[rgb]{0.50,1.00,0.58}0.728 & \cellcolor[rgb]{0.50,1.00,0.58}0.939 & \cellcolor[rgb]{0.50,1.00,0.58}0.881 & \cellcolor[rgb]{0.50,1.00,0.58}0.969 & \cellcolor[rgb]{1.00,0.88,0.30}0.636* & \cellcolor[rgb]{0.50,1.00,0.58}0.828 & \cellcolor[rgb]{0.50,1.00,0.58}0.791 & \cellcolor[rgb]{0.50,1.00,0.58}0.923 \\ 
  pmu & \cellcolor[rgb]{0.50,1.00,0.58}0.872 & \cellcolor[rgb]{0.50,1.00,0.58}0.930 & \cellcolor[rgb]{0.50,1.00,0.58}0.788 & \cellcolor[rgb]{0.50,1.00,0.58}0.898 & \cellcolor[rgb]{0.50,1.00,0.58}0.935 & \cellcolor[rgb]{0.50,1.00,0.58}0.979 & \cellcolor[rgb]{0.50,1.00,0.58}0.836 & \cellcolor[rgb]{0.50,1.00,0.58}0.903 & \cellcolor[rgb]{0.50,1.00,0.58}0.867 & \cellcolor[rgb]{0.50,1.00,0.58}0.935 \\ 
   \bottomrule
\end{tabular}
\caption{Reliability analysis of the various scales and dimensions, using Cronbach's alpha ($\alpha$) and McDonald's omega ($\omega$). Green represents a \textit{reliable} scale, while yellow with an asterisk* represents otherwise.} 
\label{tab:avantsatie_reliability}
\end{table}


==> tables/tab_subjective_comparison.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu Sep 26 11:57:45 2019
\begin{table*}[ht]
\centering
\begin{tabular}{rrllll}
  \hline
Measure Type & & ERIK-Control & EBPS-Control & Enhanced-Control & ERIK-EBPS \\ 
  \hline
  Subjective & AIL & \cellcolor[rgb]{0.50,1.00,0.58} ($t=2.23, \rho=0.033*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($t=2.13, \rho=0.042*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($t=2.36, \rho=0.026*$) &  ($t=0.25, \rho=0.808$) \\ 
  Subjective & RIM & \cellcolor[rgb]{0.50,1.00,0.58} ($U=310, \rho=0.000*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U=301, \rho=0.000*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U=610, \rho=0.000*$) &  ($U=166, \rho=0.683$) \\ 
  Subjective & RPU &  ($t=1.43, \rho=0.161$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U=273, \rho=0.007*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U=507, \rho=0.014*$) &  ($U=135, \rho=0.187$) \\ 
  Subjective & NM & \cellcolor[rgb]{0.50,1.00,0.58} ($U=248, \rho=0.048*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U=286, \rho=0.002*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U=534, \rho=0.003*$) &  ($U=136, \rho=0.193$) \\ 
  Subjective & PA & \cellcolor[rgb]{0.50,1.00,0.58} ($U=250, \rho=0.042*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($t=2.14, \rho=0.039*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U=503, \rho=0.016*$) &  ($U=208, \rho=0.436$) \\ 
  Subjective & IOS &  ($t=1.80, \rho=0.081$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U=282, \rho=0.003*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U=516, \rho=0.008*$) &  ($U=122, \rho=0.084$) \\ 
  %Subjective & RW &  ($t=0.30, \rho=0.766$) &  ($t=-0.07, \rho=0.942$) &  ($t=0.13, \rho=0.899$) &  ($t=0.33, \rho=0.743$) \\ 
  Subjective & RC & \cellcolor[rgb]{0.50,1.00,0.58} ($t=2.11, \rho=0.043*$) &  ($U=208, \rho=0.429$) &  ($U=448, \rho=0.139$) &  ($U=212, \rho=0.363$) \\ 
  %Subjective & RD &  ($U=204, \rho=0.508$) &  ($U=169, \rho=0.747$) &  ($U=372, \rho=0.851$) &  ($U=214, \rho=0.331$) \\ 
  \hline
  Subjective (sub) & ri & \cellcolor[rgb]{0.50,1.00,0.58} ($U=286, \rho=0.002*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($t=3.92, \rho=0.000*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U=582, \rho=0.000*$) &  ($U=188, \rho=0.849$) \\ 
  Subjective (sub) & rm & \cellcolor[rgb]{0.50,1.00,0.58} ($t=3.40, \rho=0.002*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($t=3.04, \rho=0.005*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($t=3.44, \rho=0.002*$) &  ($t=0.23, \rho=0.823$) \\ 
  Subjective (sub) & tp & \cellcolor[rgb]{0.50,1.00,0.58} ($U=250, \rho=0.041*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U=266, \rho=0.012*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U=517, \rho=0.008*$) &  ($U=164, \rho=0.646$) \\ 
  Subjective (sub) & tu &  ($t=0.62, \rho=0.537$) & \cellcolor[rgb]{0.50,1.00,0.58} ($t=2.37, \rho=0.024*$) &  ($t=1.61, \rho=0.115$) &  ($t=-1.39, \rho=0.175$) \\ 
  Subjective (sub) & cp & \cellcolor[rgb]{0.50,1.00,0.58} ($U=246, \rho=0.046*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U=260, \rho=0.017*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U=506, \rho=0.009*$) &  ($U=180, \rho=1.000$) \\ 
  Subjective (sub) & pmu &  ($t=1.82, \rho=0.077$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U=286, \rho=0.002*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U=529, \rho=0.005*$) &  ($U=127, \rho=0.121$) \\ 
  \hline
  Objective & WrongTotal & \cellcolor[rgb]{0.50,1.00,0.58} ($U{=}90.0, \rho{=}0.008*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U{=}93.5, \rho{=}0.011*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U{=}183.5, \rho{=}0.003*$) & ($U{=}170.5, \rho{=}0.770$) \\ 
  %Objective & WrongCold & ($U{=}128.5, \rho{=}0.129$) & ($U{=}118.0, \rho{=}0.068$) & ($U{=}246.5, \rho{=}0.053$) & ($U{=}176.5, \rho{=}0.907$) \\ 
  Objective & WrongHot & \cellcolor[rgb]{0.50,1.00,0.58} ($U{=}84.5, \rho{=}0.005*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U{=}94.0, \rho{=}0.012*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U{=}178.5, \rho{=}0.002*$) & ($U{=}173.5, \rho{=}0.840$) \\ 
  Objective & Time & ($t{=}1.676, \rho{=}0.105$) & \cellcolor[rgb]{0.50,1.00,0.58} ($t{=}2.406, \rho{=}0.022*$) & \cellcolor[rgb]{0.50,1.00,0.58} ($U{=}242.0, \rho{=}0.044*$) & ($t{=}0.257, \rho{=}0.798$) \\ 
   \hline
\end{tabular}
\caption{Results of the subjective scales and sub-dimensions, and objective measures. Green with an asterisk* marks comparisons which are significantly different. Omitted measures (RW, RD and WrongCold) do not show any significant difference.} 
\label{tab:subjective_comparison}
\end{table*}


==> tables/tab_subjective_comparison_to_median.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu Sep 26 11:57:45 2019
\begin{table}[ht]
\centering
\begin{tabular}{rcccc}
  \hline
 & ERIK-Random & Control-Random & EBPS-Random & Enhanced-Random \\ 
  \hline
AIL & \cellcolor[rgb]{0.50,1.00,0.58} + &  = & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + \\ 
  RIM & \cellcolor[rgb]{0.50,1.00,0.58} + &  = & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + \\ 
  RPU & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + \\ 
  NM & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + \\ 
  PA &  = &  = & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + \\ 
  IOS &  = &  = & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + \\ 
  RW & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + &  = & \cellcolor[rgb]{0.50,1.00,0.58} + \\ 
  RC & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + \\ 
  RD & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + \\ 
  ri & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{1.00,0.88,0.30} - & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + \\ 
  rm & \cellcolor[rgb]{0.50,1.00,0.58} + &  = & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + \\ 
  tp & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + \\ 
  tu &  = &  = & \cellcolor[rgb]{0.50,1.00,0.58} + &  = \\ 
  cp & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + \\ 
  pmu & \cellcolor[rgb]{0.50,1.00,0.58} + &  = & \cellcolor[rgb]{0.50,1.00,0.58} + & \cellcolor[rgb]{0.50,1.00,0.58} + \\ 
   \hline
\end{tabular}
\caption{Results of the comparison of means to the scale's median value on each of the subjective measures. Green + (plus) marks greater than median, Yellow - (minus) marks lower than median, and = (equal) marks not significantly different from the median.} 
\label{tab:subjective_comparison_to_median}
\end{table}


==> tables/tab_subjective_shapiro_wilk.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Thu Sep 26 11:57:45 2019
\begin{table}[ht]
\centering
\begin{tabular}{rllll}
  \hline
 & C-ERIK & C-Control & C-EBPS & C-Enhanced \\ 
  \hline
AIL & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.219$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.080$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.550$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.056$ \\ 
  RIM & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.006*$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.943$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.037*$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.001*$ \\ 
  RPU & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.050$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.767$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.030*$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.004*$ \\ 
  NM & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.027*$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.271$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.013*$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.002*$ \\ 
  PA & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.030*$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.557$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.557$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.029*$ \\ 
  IOS & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.279$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.202$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.023*$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.007*$ \\ 
  RW & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.576$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.989$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.477$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.848$ \\ 
  RC & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.176$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.478$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.005*$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.000*$ \\ 
  RD & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.013*$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.001*$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.059$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.001*$ \\ 
  ri & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.027*$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.120$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.163$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.003*$ \\ 
  rm & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.550$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.640$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.251$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.066$ \\ 
  tp & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.001*$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.399$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.000*$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.000*$ \\ 
  tu & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.499$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.326$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.771$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.472$ \\ 
  cp & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.000*$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.004*$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.000*$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.000*$ \\ 
  pmu & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.121$ & \cellcolor[rgb]{0.50,1.00,0.58} $\rho=0.739$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.006*$ & \cellcolor[rgb]{1.00,0.88,0.30} $\rho=0.004*$ \\ 
   \hline
\end{tabular}
\caption{Results of the Shapiro-Wilk's test of normality on each of the subjective measures. Green marks data which are normally distributed; Yellow with an asterisk* marks otherwise.} 
\label{tab:subjective_shapiro_wilk}
\end{table}

